Donaldson-Thomas Transformation of Double Bruhat Cells in General Linear Groups

Kontsevich and Soibelman defined the Donaldson-Thomas invariants of a 3d Calabi-Yau category with a stability condition. Any cluster variety can produce an example of such a category, whose corresponding Donaldson-Thomas invariants are encoded by a special formal automorphism of the cluster variety, known as the Donaldson-Thomas transformation. In this paper we prove a conjecture of Goncharov and Shen in the case of $\mathrm{GL}_n$, which describes the Donaldson-Thomas transformation of the double quotient of the double Bruhat cells $H \backslash \mathrm{GL}_n^{u,v}/H$ where $H$ is a maximal torus, as a certain explicit cluster transformation related to Fomin-Zelevinsky's twist map. Our result, combined with the work of Gross, Hacking, Keel, and Kontsevich, proves the duality conjecture of Fock and Goncharov in the case of $H\backslash \mathrm{GL}_n^{u,v}/H$.

==> scratch.tex <==
Next we will give a more pictorial construction of constructing the greedy and anti-greedy reduced words of a Weyl group element $w$ using combinatorics. Draw an grid with $n$ horizontal lines and $n$ vertical lines, and label the horizontal lines from top to bottom, the vertical lines from right to left, by integers $1,\dots, n$ respectively. Let $(i,j)$ denote the intersection between the $i$th vertical line and the $j$th horizontal line. On such grid, mark all intersections of the form $(w(i),i)$. There are in total $n$ such intersections, with one on each horizontal line and one on each vertical line. Now draw $\daleth$-shaped curves with red color on this grid by first going along each horizontal line from left to right, turn right at the marked intersection, and then go straight down; also draw L-shaped curves with blue color on this grid by first going along each horizontal line from right to left, turn right at the marked intersection, and then go straight up. 

We claim that the red color curves give rise to the greedy reduced word of $w$ and the blue curves give rise to the anti-greedy reduced word of $w$. Let's describe the process to extract the actual greedy reduced word from the red curves. Note that these red curves intersect at precisely $l(w)$ many intersections, each of which will give rise to a letter in the greedy reduced word. To determine these letters, we do the following:
\begin{enumerate}
    \item go along the red curve starting from $i$ on the left side of the grid and zig-zag between intersection points of red curves;
    \item as a result, you get $n$ paths going from northwest to southeast, each of which goes from the label $i$ on the left hand side of the grid to the label $i$ on the bottom of the grid; call the path going from $i$ to $i$ the $i$th path;
    \item an intersection between two red curves corresponds to the letter $i$ if it lies between the $i$th path and the $(i+1)$th path;
    \item assemble these letters in by going from northwest to southeast again; whenever there is an ambiguity of the order of two letters, the larger one always goes first.
\end{enumerate}
An analogous algorithm can be deduced for getting the anti-greedy word from the blue curves:
\begin{enumerate}
    \item go along the blue curve starting from $i$ on the right side of the grid and zig-zag between intersection points of blue curves;
    \item as a result, you get $n$ paths going from southeast to northwest, each of which goes from the label $i$ on the right hand side of the grid to the label $i$ on the top of the grid; call the path going from $i$ to $i$ the $i$th path;
    \item an intersection between two red curves corresponds to the letter $i$ if it lies between the $i$th path and the $(i+1)$th path;
    \item assemble these letters in by going from southeast to northwest again; whenever there is an ambiguity of the order of two letters, the smaller one always goes first.
\end{enumerate}

\begin{exmp} Let's apply this pictorial method to determine the greedy reduced word and the anti-greedy reduced word for the permutation $w=\begin{pmatrix} 1 & 2 & 3 & 4 \\ 4 & 2 & 1 & 3\end{pmatrix}$. First we draw a $4\times 4$ grid, label the mark intersections, and draw the red curves and blue curves as follows.
\[
\tikz{
\draw[ultra thick, red] (0,1) -- (2,1) -- (2,0);
\draw[ultra thick, red] (0,2) -- (4,2) -- (4,0);
\draw[ultra thick, red] (0,3) -- (3,3) -- (3,0);
\draw[ultra thick, red] (0,4) -- (1,4) -- (1,0);
\draw[ultra thick, blue] (5,1) -- (2,1) -- (2,5);
\draw[ultra thick, blue] (5,2) -- (4,2) -- (4,5);
\draw[ultra thick, blue] (5,3) -- (3,3) -- (3,5);
\draw[ultra thick, blue] (5,4) -- (1,4) -- (1,5);
\node at (1,4) [] {$\times$};
\node at (3,3) [] {$\times$};
\node at (4,2) [] {$\times$};
\node at (2,1) [] {$\times$};
\node at (0,1) [left] {$4$};
\node at (0,2) [left] {$3$};
\node at (0,3) [left] {$2$};
\node at (0,4) [left] {$1$};
\node at (5,1) [right] {$4$};
\node at (5,2) [right] {$3$};
\node at (5,3) [right] {$2$};
\node at (5,4) [right] {$1$};
\node at (1,0) [below] {$4$};
\node at (2,0) [below] {$3$};
\node at (3,0) [below] {$2$};
\node at (4,0) [below] {$1$};
\node at (1,5) [above] {$4$};
\node at (2,5) [above] {$3$};
\node at (3,5) [above] {$2$};
\node at (4,5) [above] {$1$};
}
\]
Next we separate the red curves and the blue curves, and use the algorthms above to determine the greedy and anti-greedy reduced words.
\[
\tikz{
\draw[ultra thick, red] (0,1) -- (2,1) -- (2,0);
\draw[ultra thick, red] (0,2) -- (4,2) -- (4,0);
\draw[ultra thick, red] (0,3) -- (3,3) -- (3,0);
\draw[ultra thick, red] (0,4) -- (1,4) -- (1,0);
\node at (0,1) [left] {$4$};
\node at (0,2) [left] {$3$};
\node at (0,3) [left] {$2$};
\node at (0,4) [left] {$1$};
\node at (1,0) [below] {$4$};
\node at (2,0) [below] {$3$};
\node at (3,0) [below] {$2$};
\node at (4,0) [below] {$1$};
}
\quad \quad \quad \quad 
\tikz{
\draw[ultra thick, red] (0,1) -- (0.9,1) -- (1,0.9) -- (1,0); 
\draw[ultra thick, red] (0,2) -- (0.9,2) -- (1,1.9) -- (1,1.1)--(1.1,1) -- (2,1) -- (2,0);
\draw[ultra thick, red] (0,3) -- (0.9,3) -- (1,2.9) -- (1,2.1) -- (1.1,2) -- (2.9,2) -- (3,1.9) -- (3,0);
\draw[ultra thick, red] (0,4) -- (1,4) -- (1,3.1) -- (1.1,3) -- (3,3) -- (3,2.1) -- (3.1,2) -- (4,2) -- (4,0);
\node at (0,1) [left] {$4$};
\node at (0,2) [left] {$3$};
\node at (0,3) [left] {$2$};
\node at (0,4) [left] {$1$};
\node at (1,0) [below] {$4$};
\node at (2,0) [below] {$3$};
\node at (3,0) [below] {$2$};
\node at (4,0) [below] {$1$};
\node at (1,3) [below right] {$s_1$};
\node at (1,2) [below right] {$s_2$};
\node at (1,1) [below right] {$s_3$};
\node at (3,2) [below right] {$s_1$};
}
\]
\[
\tikz{
\draw[ultra thick, blue] (5,1) -- (2,1) -- (2,5);
\draw[ultra thick, blue] (5,2) -- (4,2) -- (4,5);
\draw[ultra thick, blue] (5,3) -- (3,3) -- (3,5);
\draw[ultra thick, blue] (5,4) -- (1,4) -- (1,5);
\node at (5,1) [right] {$4$};
\node at (5,2) [right] {$3$};
\node at (5,3) [right] {$2$};
\node at (5,4) [right] {$1$};
\node at (1,5) [above] {$4$};
\node at (2,5) [above] {$3$};
\node at (3,5) [above] {$2$};
\node at (4,5) [above] {$1$};
} \quad \quad \quad \quad
\tikz{
\draw[ultra thick, blue] (5,1) -- (2,1) -- (2,3.9) -- (1.9,4) -- (1,4) -- (1,5);
\draw[ultra thick, blue] (5,2) -- (4,2) -- (4,2.9) -- (3.9,3) -- (3,3) -- (3,3.9) -- (2.9,4) -- (2.1,4) -- (2,4.1) -- (2,5);
\draw[ultra thick, blue] (5,3) -- (4.1,3) -- (4,3.1) -- (4,3.9) -- (3.9,4) -- (3.1,4) -- (3,4.1) -- (3,5);
\draw[ultra thick, blue] (5,4) -- (4.1,4) -- (4,4.1) -- (4,5);
\node at (5,1) [right] {$4$};
\node at (5,2) [right] {$3$};
\node at (5,3) [right] {$2$};
\node at (5,4) [right] {$1$};
\node at (1,5) [above] {$4$};
\node at (2,5) [above] {$3$};
\node at (3,5) [above] {$2$};
\node at (4,5) [above] {$1$};
\node at (4,4) [below right] {$s_1$};
\node at (4,3) [below right] {$s_2$};
\node at (3,4) [below right] {$s_2$};
\node at (2,4) [below right] {$s_3$};
}
\]
Thus the corresponding greedy and anti-greedy reduced words are
\[
\vec{i}_w=(1,2,3,1) \quad \quad \text{and} \quad \quad \vec{i}^*_w=(2,1,2,3).
\]
\end{exmp}

From the construction of cluster structures on double Bruhat cells, we see that if two reduced words differ by swapping two adjacent letters that differ more than 1, neither the resulting cluster seed tori nor maps between cluster seed tori and double Bruhat cells change. Thus it is convenient to introduce the following equivalence relation.

\begin{defn} Two reduced words of the same Weyl group element is said to be \textit{equivalent} if one can be obtained from the other via a sequence of \textit{equivalence moves}, each of which interchanges two adjacent letters differ more than 1:
\[
(\dots, i,j,\dots) \rightsquigarrow (\dots, j,i,\dots) \quad \quad \quad \text{if $|i-j|>1$.}
\]
We denote two equivalent reduced words $\vec{i}$ and $\vec{i}'$ of $w$ by $\vec{i}\sim \vec{i}'$.
\end{defn}

\begin{prop} For any Weyl group element $w$, $\vec{i}_w\sim \vec{i}_{w^{-1}}^\circ$ and $\vec{i}_w^* \sim \left(\vec{i}_{w^{-1}}^*\right)^\circ$.
\end{prop}
\begin{proof} Note that picture associated to $w^{-1}$ (the $n\times n$ grid with marked intersections, red curves, and blue curves) can be obtained from the one of $w$ by flipping over the northeast-southwest diagonal. There is never ambiguity between the order of two letters differ by 1. Thus taking the opposite reduced words of $\vec{i}_{w^{-1}}$ and $\vec{i}_{w^{-1}}^*$ restores the greedy and anti-greedy reduced words of $w$ up to equivalence.
\end{proof}

\begin{defn} For a pair of Weyl group elements $(u,v)$, we define its greedy reduced word to be $\vec{i}_{(u,v)}=\vec{i}_u\#\vec{i}_v$ and its anti-greedy reduced word to be $\vec{i}^*_{(u,v)}=\vec{i}_v^*\#\vec{i}_u^*$.
\end{defn}

In fact, the greedy and anti-greedy reduced words of a pair of Weyl group elements can be put together into one picture as we did for a single Weyl group element:9 just draw the picture associated to $u$ and the picture associated to $v$ and put them diagonally together. For example, the following picture is associated to the pair of Weyl group elements $(u,v)$ where
\[
u=\begin{pmatrix} 1 & 2 & 3 & 4 \\ 4 & 2 & 1 & 3\end{pmatrix} \quad \quad \text{and} \quad \quad v=\begin{pmatrix} 1 & 2 & 3 & 4 \\  3 & 1 & 4 & 2 \end{pmatrix}
\]
\[
\tikz{
\draw[ultra thick, red] (0,1) -- (2,1) -- (2,-1.5) to [out=-90,in=180] (2.5,-2) -- (5,-2) -- (5,-4);
\draw[ultra thick, red] (0,2) -- (4,2) -- (4,0.5) to [out=-90,in=180] (4.5,0) -- (6,0) -- (6,-4);
\draw[ultra thick, red] (0,3) -- (3,3) -- (3,-0.5) to [out=-90,in=180] (3.5,-1) -- (8,-1) -- (8,-4);
\draw[ultra thick, red] (0,4) -- (1,4) -- (1,-2.5) to [out=-90,in=180] (1.5,-3) -- (7,-3) -- (7,-4);
\draw[ultra thick, blue] (2,5) -- (2,1) -- (4.5,1) to [out=0,in=90] (5,0.5) -- (5,-2) -- (9,-2);
\draw[ultra thick, blue] (4,5) -- (4,2) -- (5.5,2) to [out=0,in=90] (6,1.5) -- (6,0) -- (9,0);
\draw[ultra thick, blue] (3,5) -- (3,3) -- (6.5,3) to [out=0, in=90] (7,2.5) -- (7,-3) -- (9,-3);
\draw[ultra thick, blue] (1,5) -- (1,4) -- (7.5,4) to [out=0,in=90] (8,3.5) -- (8,-1) -- (9,-1);
\node at (1,4) [] {$\times$};
\node at (3,3) [] {$\times$};
\node at (4,2) [] {$\times$};
\node at (2,1) [] {$\times$};
\node at (6,0) [] {$\times$};
\node at (5,-2) [] {$\times$};
\node at (8,-1) [] {$\times$};
\node at (7,-3) [] {$\times$};
\node at (0,1) [left] {$4$};
\node at (0,2) [left] {$3$};
\node at (0,3) [left] {$2$};
\node at (0,4) [left] {$1$};
\node at (9,-3) [right] {$4$};
\node at (9,-2) [right] {$3$};
\node at (9,-1) [right] {$2$};
\node at (9,0) [right] {$1$};
\node at (8,-4) [below] {$4$};
\node at (7,-4) [below] {$3$};
\node at (6,-4) [below] {$2$};
\node at (5,-4) [below] {$1$};
\node at (1,5) [above] {$4$};
\node at (2,5) [above] {$3$};
\node at (3,5) [above] {$2$};
\node at (4,5) [above] {$1$};
}
\]

\begin{prop} The boundary-removed quiver $\vec{i}_{(u,v)}$ associated to the greedy reduced word of $(u,v)$ is isomorphic to the boundary-removed quiver $\vec{i}^*_{(u,v)}$ associated to the anti-greedy reduced word of $(u,v)$.
\end{prop}
